Uniform spanning forest on the integer lattice with drift in one coordinate

In this article we investigate the Uniform Spanning Forest ($\mathsf{USF}$) in the nearest-neighbour integer lattice $\mathbf{Z}^{d+1} = \mathbf{Z}\times \mathbf{Z}^d$ with an assignment of conductances that makes the underlying (Network) Random Walk ($\mathsf{NRW}$) drifted towards the right of the first coordinate. This assignment of conductances has exponential growth and decay; in particular, the measure of balls can be made arbitrarily close to zero or arbitrarily large. We establish upper and lower bounds for its Green's function. We show that in dimension $d = 1, 2$ the $\mathsf{USF}$ consists of a single tree while in $d \geq 3,$ there are infinitely many trees. We then show, by an intricate study of multiple $\mathsf{NRW}$s, that in every dimension the trees are one-ended; the technique for $d = 2$ is completely new, while the technique for $d \geq 3$ is a major makeover of the technique for the proof of the same result for the graph $\mathbf{Z}^d.$ We finally establish the probability that two or more vertices are $\mathsf{USF}$-connected and study the distance between different trees.

==> PhDHarmonicDirichlet.tex <==
\chapter{The spaces $\dirichlet$ and $\harDirichlet$}\label{Annex: Harmonic Dirichlet functions}
We study further the spaces $\dirichlet$ and $\harDirichlet$ (\ref{Equation: Definition of the spaces D and HD}) in order to provide conditions under which $\nabla \harDirichlet = \{0\}.$ Since we are going to be investigating properties of harmonic functions, recall the definition of the transition operator (\ref{Equation: Definition of transition operator}) and its main properties (\ref{Proposition: Properties of the transition operator}).

Recall from Annex \ref{Annex: Electrical Networks} what does it mean for a network $\Gamma = (\strG, c),$ $\strG = (\strV, \strE),$ to satisfy the usual assumptions. Fix such a network throughout this Annex; no other networks will be considered.

	Most of the work in this chapter is based on \cite{Barlow:RWHK} and \cite{Soardi:PTIN} with the necessary adaptations to our case; in particular, we do not assume locally finiteness of the underlying graph. 

	\section{The topological spaces $\dirichlet$ and $\harDirichlet.$}
	Consider a vertex $o$ of $\Gamma.$ We introduce the following inner product on $\dirichlet$ which depend on $o,$
	\begin{equation}\label{Equation: Definition of the inner product in the Dirichlet space}
		\begin{split}
			\prodEsc{f}{g}_o &= f(o) g(o) + \prodEsc{\nabla f}{\nabla g}_{\ell_-^2(\strE; r)}, \\
			\norm{f}_o^2 &= \prodEsc{f}{f}_o = f(o)^2 + \energyDir{f}.
		\end{split}
	\end{equation}
	It is easy to check that $(f, g) \mapsto \prodEsc{f}{g}_o$ defines an inner product, except perhaps for the detail in proving that $\prodEsc{f}{f}_o = 0$ is sufficient for $f = 0.$ To see this observe that $\prodEsc{f}{f}_o = 0$ implies $f(o) = 0$ and $\nabla f = 0,$ the second of these relations implies $f(e^+) = f(e^-)$ for every edge $e$ with $c(e) > 0.$ Since the random walk is irreducible, for every vertex $v,$ there exists a path $\gamma$ of positive-conductance edges with $\gamma^- = o$ and $\gamma^+ = v,$ thus $f(o) = f(v).$ Incidentally, we showed
	\begin{Proposition}\label{Proposition: A function is constant iff its energy is zero}
		For a function $f:\strV \to \R$ to be constant it is necessary and sufficient that $\energyDir{f} = 0.$ Furthermore, if $f$ is constant and $\varphi:\strV \to \R$ is any function, $\energyDir{f + \varphi} = \energyDir{\varphi}.$
	\end{Proposition}
	The previous inner product depends on the choosing of the vertex $o,$ however, \emph{the topology it defines is independent of the choice of $o.$} To see this, consider any other vertex $o'.$ We will show that there exist constants $c, C > 0$ such that for every function $f \in \dirichlet,$ we have
	\begin{displaymath}
		c \norm{f}_o \leq \norm{f}_{o'} \leq C \norm{f}_o. 
	\end{displaymath}
	This will prove that the two normed spaces $(\dirichlet, \norm{\cdot}_o)$ and $(\dirichlet, \norm{\cdot}_{o'})$ possess the same topology. By symmetry, suffices to show the inequality $\norm{f}_{o'} \leq C \norm{f}_o.$ To show it, consider a minimal length path $(e_j)_{1 \leq j \leq m}$ from $o$ to $o'$ whose edges all have positive conductances (this is possible due to irreducibility of the random walk). By minimality, the edges are not repeated. The Cauchy-Schwarz inequality applied to the coefficients 1, $\sqrt{r(e_1)}, \ldots, \sqrt{r(e_m)},$ gives
	\begin{align*}
		f(o')^2 &= \left[ f(o) + \sum_{j = 1}^m \sqrt{r(e_j)} \left( \sqrt{c(e_j)} \big( f(e_j^+) - f(e_j^-) \big) \right) \right]^2 \\
		&\leq \left[ 1 + \sum_{j = 1}^m r(e_j) \right] \left[ f(o)^2 + \sum_{j = 1}^m c(e_j) \big( f(e_j^+) - f(e_j^-) \big)^2 \right] \\
		&\leq \left[ 1 + \sum_{j = 1}^m r(e_j) \right] \left[ f(o)^2 + \energyDir{f} \right] = c \norm{f}_o^2.
	\end{align*}
	This inequality is important in its own.
	\begin{Proposition}\label{Proposition: Evaluation is a continuous linear function on the Dirichlet space}
		For each vertex $v \in \strV$ there exists a constant $c = c_v > 0$ such that $|f(v)| \leq c \norm{f}_o,$ that is to say, the function $f \mapsto f(v)$ from $\dirichlet$ into $\R$ is linear and continuous. Thus, evaluations on $\dirichlet$ are continuous linear forms.
	\end{Proposition}

	We are also interested in $\harDirichlet.$ From (\ref{Remark: A function is harmonic iff the divergence of its gradient is zero}), $\harDirichlet$ is the set of function $f$ such that
	\begin{displaymath}
		\diver \nabla f = f - Pf = 0.
	\end{displaymath}
	Since $\nabla$ can be thought as a function $\dirichlet \to \ell_-^2(\strE; r)$ and $\diver:\ell_-^2(\strE; r) \to \ell^2(\strV; c),$ we reach that $\diver \circ \nabla:\dirichlet \to \ell^2(\strV; c)$ and $\harDirichlet$ is the kernel of this linear function. Furthermore, by (\ref{Equation: Operator norms of the divergence and gradient}), we know
	\begin{displaymath}
		\norm{\diver \nabla f}_{\ell^2(\strV; c)} \leq \sqrt{2} \norm{\nabla f}_{\ell_-^2(\strE; r)} = \sqrt{2} \energyDir{f}.
	\end{displaymath}
	We have established the following proposition.
	\begin{Proposition}\label{Proposition: I-P maps D into L2}
		Denote by $I_\dirichlet$ the identity function in $\dirichlet.$ Then $I_\dirichlet - P = \diver \circ \nabla:\dirichlet \to \ell^2(\strV; c)$ is a continuous linear function satisfying that, for every function $f \in \dirichlet,$
		\begin{displaymath}
			\norm{f - Pf}_{\ell^2(\strV; c)}^2 \leq 2 \energyDir{f} \leq 2 \norm{f}_o.
		\end{displaymath}
		Furthermore, $\harDirichlet$ is the kernel of $I_\dirichlet - P.$
	\end{Proposition}
	In particular, $I_\dirichlet - P$ is a continuous linear function $\dirichlet \to \ell^2(\strV; c)$ whose operator norm is bounded from above by $\sqrt{2},$ regardless of the choice of norm in $\dirichlet.$

	In a similar manner, the definitions of the norms in $\dirichlet$ and $\ell_-^2(\strE; r)$ has the following corollary. The gradient $\nabla:\dirichlet \to \ell_-^2(\strE; r)$ satisfies, for every $f \in \dirichlet,$
	\begin{equation}\label{Equation: The gradient is continuous from the Dirichlet into the flows}
		\norm{\nabla f}_{\ell_-^2(\strE; r)} \leq \norm{f}_o.
	\end{equation}
	In other words, $\nabla$ is a continuous linear function with norm $\leq 1$ when viewed $\dirichlet \to \ell_-^2(\strE; r),$ regardless of the choice of norm in $\dirichlet.$

	\begin{Proposition}\label{Proposition: Characterisation of the topology in the Dirichlet space}
		The inner product (\ref{Equation: Definition of the inner product in the Dirichlet space}) defines a structure of Hilbert space on $\dirichlet;$ the topology of this structure is independent of the choice of $o.$ For a sequence $(f_n)$ in $\dirichlet$ to converge to $f \in \dirichlet$ it is necessary and sufficient that $\nabla f_n \to \nabla f$ in $\ell_-^2(\strE; r)$ and $f_n(o) \to f(o)$ in $\R$ for some vertex $o;$ equivalently, for $(f_n)$ to converge to $f$ in the topology of $\dirichlet$ it is necessary and sufficient that $\energyDir{f - f_n} \to 0$ and $f_n(o) \to f(o)$ (convergences in $\R$) for some vertex $o.$ Furthermore, the subspace $\harDirichlet$ is closed in $\dirichlet.$
	\end{Proposition}
	\begin{proof}
		We already proved that (\ref{Equation: Definition of the inner product in the Dirichlet space}) defines an inner product and the topology its norm defines does not depend on $o.$ We now prove $\dirichlet$ is complete with respect to (any of) the norm(s) $\norm{f}_o.$ Since
		\begin{displaymath}
			\norm{f}_o^2 = f(o)^2 + \energyDir{f} = f(o)^2 + \energyFlow{\nabla f}^2,
		\end{displaymath}
		it follows readily that $f_n \to f$ in $\dirichlet$ is equivalent to $f_n(o) \to f(o)$ and $\nabla f_n \to \nabla f,$ which in turn is the same as saying $f_n(o) \to f(o)$ and $\energyDir{f - f_n} \to 0.$
		
		We now prove $\dirichlet$ is a complete space. Consider a sequence $(f_n)$ that is fundamental in $\dirichlet$ with respect to $\norm{ \cdot }_o;$ that is to say, the sequence $\ds \left( \sup_{m \geq n} \norm{f_n - f_m}_o \right)_{n \in \N}$ tends to zero in $\R.$ The definition of the norm $\norm{\cdot}_o$ shows at once that $(f_n(o))$ is a fundamental sequence in $\R,$ hence convergent to some $\lambda,$ and $(\nabla f_n)$ is fundamental in $\ell_-^2(\strE; r),$ hence converging to some $\theta$ since $\ell_-^2(\strE; r)$ is also complete. By (\ref{Proposition: The orthogonal space to the cycles are the flows with potential}), it follows that $\nabla f_n \in \lozenge^\perp$ and this a closed subspace, hence the limit of $\nabla f_n$ belongs to $\lozenge^\perp.$ Therefore, $\theta = \nabla g$ for some $g \in \dirichlet.$ Let $f = g + \lambda - g(o),$ where $\lambda$ and $g(o)$ denote constant functions. Then $f_n(o) \to f(o)$ and $\energyDir{f_n - f} = \energyDir{f_n - g} \to 0$ by (\ref{Proposition: A function is constant iff its energy is zero}). Therefore, $f_n \to f$ in $\dirichlet.$
		
		Finally, $\harDirichlet$ is closed since it is the kernel of a continuous linear function (\ref{Proposition: I-P maps D into L2}).
	\end{proof}

	\section{Convergence in $\dirichlet.$}
	In the previous proposition, the topology of $\dirichlet$ was characterised as two convergences in $\R,$ one of them being that of the Dirichlet energy. We proceed to develop a few tools in regards to this energy.
	\begin{Proposition}\label{Proposition: Lipschitz functions preserve Dirichlet functions}
		Suppose $\strI$ is an interval in $\R,$ $\lambda > 0$ and that $\varphi:\strI \to \R$ is a $\lambda$-Lipschitz function, that is to say, $|\varphi(s) - \varphi(t)| \leq \lambda |s - t|$ for all $s, t \in \strI.$ For every Dirichlet function $h$ such that $h(\strV) \subset \strI,$ the compound function $\varphi \circ h$ also belongs to $\dirichlet$ and it satisfies $\energyDir{\varphi \circ h} \leq \lambda^2 \energyDir{h}.$
	\end{Proposition}
	\begin{proof}
		Expanding the definition of $\energyDir{\varphi \circ h}$ we use the Lipschitz condition and the result is immediate.
	\end{proof}
	
	\begin{Proposition}\label{Proposition: The Dirichlet energy of the difference of two functions is greater than the Dirichlet energy of the difference of any of them minus its minimum}
		Let $f, g$ be two functions defined on $\strV.$ Set $\varphi = \min(f, g)$ and $\psi = \max(f, g).$ Then, for all pair of vertices $x, y,$
		\begin{displaymath}
			|f(x) - \varphi(x) - f(y) + \varphi(y)| \leq |f(x) - g(x) - f(y) + g(y)|,
		\end{displaymath}
		and
		\begin{displaymath}
			|f(x) - \psi(x) - f(y) + \psi(y)| \leq |f(x) - g(x) - f(y) + g(y)|.
		\end{displaymath}
		In particular,
		\begin{displaymath}
			\energyDir{f - \varphi} \leq \energyDir{f - g} \quad \text{ and } \quad \energyDir{f - \psi} \leq \energyDir{f - g}.
		\end{displaymath}
	\end{Proposition}
	\begin{proof}
		The case of $\psi$ is proven with obvious modification to the case of $\varphi,$ and we will show only the latter. By symmetry between the pairs of $x$ and $y,$ and $f$ and $g,$ there are three cases to consider. In the first case, $\varphi(x) = f(x)$ and $\varphi(y) = f(y),$ and in the second, $\varphi(x) < f(x)$ and $\varphi(y) < f(y),$ but in any of these, the result is obvious. In the third case, $\varphi(x) = f(x)$ and $\varphi(y) < f(y),$ but then $f(x) \leq g(x)$ and $\varphi(y) = g(y),$ implying
		\begin{align*}
			|f(x) - \varphi(x) - f(y) + \varphi(y)| &= f(y) - g(y) \\
			&\leq f(y) - g(y) + g(x) - f(x) \\
			&= |f(y) - g(y) - f(x) + g(x)|.
		\end{align*}
		The last part follows upon noticing that
		\begin{align*}
			\energyDir{f - \varphi} &= \sum_{e \in \strE} \dfrac{1}{2} c(e) \big( f(e^-) - \varphi(e^-) - f(e^+) + \varphi(e^+) \big)^2 \\
			&\leq \sum_{e \in \strE} \dfrac{1}{2} c(e) \big( f(e^-) - g(e^-) - f(e^+) + g(e^+) \big)^2 = \energyDir{f - g},
		\end{align*}
		which is the desired inequality.
	\end{proof}
	
	We introduce the common notation $t^+ = \max(t, 0)$ for $t \in \R;$ we set $f^+$ to be the function $x \mapsto f(x)^+$ and $t^- = (-t)^+$ and $f^- = (-f)^+.$ The functions $f^+$ and $f^-$ are often referred to as the \emph{positive} and \emph{negative} part of $f,$ respectively. Despite the name, $f^- \geq 0.$
	
	\begin{Proposition}\label{Proposition: The Dirichlet energy of the positive and negative parts of a function}
		For any pair of functions $f, g:\strV \to \R,$ we have the inequalities
		\begin{displaymath}
			\energyDir{f^+ - g^+} + \energyDir{f^- - g^-} \leq \energyDir{f - g} \leq 2\energyDir{f^+ - g^+} + 2\energyDir{f^- - g^-}.
		\end{displaymath}
	\end{Proposition}
	\begin{proof}
		Observe first that
		\begin{displaymath}
			(t - s)^2 = (t^+ - s^+)^2 + (t^- - s^-)^2 - 2(t^+ - s^+)(t^- - s^-) \geq (t^+ - s^+)^2 + (t^- - s^-)^2
		\end{displaymath}
		since $(t^+ - s^+)(t^- - s^-) \geq 0;$ we also have the inequality
		\begin{displaymath}
			(t - s)^2 \leq 2(t^+ - s^+)^2 + 2(t^- - s^-)^2,
		\end{displaymath}
		which follows from $(a + b)^2 \leq 2a^2 + 2b^2.$
	\end{proof}
	
	\begin{Proposition}\label{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}
		For a function $f$ to belong to $\dirichlet$ it is necessary and sufficient that its positive and negative parts should belong to $\dirichlet.$ Moreover, for a sequence $(f_n)$ in $\dirichlet$ to converge to some $f \in \dirichlet$ it is necessary and sufficient that the sequences $(f_n^+)$ and $(f_n^-)$ converge to $f^+$ and $f^-$ in $\dirichlet,$ respectively.
	\end{Proposition}
	\begin{proof}
		By (\ref{Proposition: The Dirichlet energy of the positive and negative parts of a function}), $f \in \dirichlet \iff f^\pm \in \dirichlet.$ Next, it is clear that $f_n^\pm(o) \to f^\pm(o)$ and again (\ref{Proposition: The Dirichlet energy of the positive and negative parts of a function}) applied to $g = f_n$ shows that $\energyDir{f - f_n} \to 0$ is the same as saying that both $\energyDir{f^\pm - f_n^\pm} \to 0.$ The conclusion follows from the characterisation of convergence in $\dirichlet$ given by (\ref{Proposition: Characterisation of the topology in the Dirichlet space}).
	\end{proof}

	\section{The topological space $\dirichlet_0.$}
	Let $\dirichlet_0$ be the closure in $\dirichlet$ of the set of Dirichlet functions with finite support, in other words,
	\begin{equation}\label{Equation: Definition of D0}
		\begin{split}
			\compactSupp[_\R]{\strV} &= \{f:\strV \to \R \mid f \text{ has finite support}\}, \\
			\dirichlet_0 &= \closure{\compactSupp[_\R]{\strV}}.
		\end{split}
	\end{equation}
	Clearly, $\compactSupp[_\R]{\strV}$ is a vector subspace of $\dirichlet$ and it is a well-known fact from linear algebra that the closure, relative to a norm, of a vector subspace is also a vector subspace. Furthermore, $\dirichlet_0$ being closed in the complete space $\dirichlet,$ is complete in and of itself. Thus, we reach the following result.
	\begin{Proposition}\label{Proposition: D0 is a Hilbert space}
		$\dirichlet_0$ is a Hilbert space for any choice of norm $\norm{\cdot}_o.$
	\end{Proposition}

	\begin{Proposition}
		We have $\ell^2(\strV; c) \subset \dirichlet_0;$ furthermore, if a sequence $f_n \in \ell^2(\strV; c)$ converges to $f$ in $\ell^2(\strV; c),$ then $f_n$ converges to $f$ in $\dirichlet_0.$
	\end{Proposition}
	\begin{proof}
		The inequality
		\begin{displaymath}
			|f_n(x) - f(x)| \leq c(x)^{-1} \norm{f_n - f}_{\ell^2(\strV; c)}
		\end{displaymath}
		shows that evaluation at $x,$ $f \mapsto f(x),$ is a continuous linear form on $\ell^2(\strV; c).$ Also, the inequality (\ref{Proposition: The square integrable functions are Dirichlet}) shows that if $\norm{f_n - f}_{\ell^2(\strV; c)} \to 0,$ then $\energyDir{f_n - f} \to 0.$ Therefore, if $f_n \to f$ in $\ell^2(\strV; c)$ then $f_n \to f$ in $\dirichlet.$ Thus, suffices to show \emph{$\compactSupp[_\R]{\strV}$ is dense in $\ell^2(\strV; c)$ relative to the topology of $\ell^2(\strV; c)$}. Consider $(\strV_n)$ an increasing sequence of finite sets such that $\strV_n \uparrow \strV.$ If $f \in \ell^2(\strV; c),$ then $f \indic{\strV_n} \to f$ and $|f \indic{\strV_n}| \leq |f|,$ so the Lebesgue's dominated convergence theorem shows that every function in $\ell^2(\strV; c)$ is the limit of functions with finite support, in other words $\compactSupp[_\R]{\strV}$ is dense in $\ell^2(\strV; c)$ in this space.
	\end{proof}
	
	\begin{Proposition}\label{Proposition: Gauss Green for finite support and dirichlet functions}
		Let $f \in \dirichlet$ and $\varphi \in \ell^2(\strV; c).$ Then $f- Pf$ is square integrable (\ref{Proposition: I-P maps D into L2}) and
		\begin{displaymath}
			\prodEsc{\nabla f}{\nabla \varphi}_{\ell_-^2(\strE; r)} = \prodEsc{f - Pf}{\varphi}_{\ell_-^2(\strE; r)},
		\end{displaymath}
		(``Gauss-Green formula''). The formula may fail if $f$ and $\varphi$ are only assumed in the space $\dirichlet_0.$
	\end{Proposition}
	\begin{proof}
		We may apply (\ref{Proposition: The gradient and divergence are adjoint}) to $\nabla f \in \ell_-^2(\strE; r)$ and $\varphi \in \ell^2(\strV; c).$ Bearing in mind $\diver \circ \nabla = I_\dirichlet - P,$ the result follows.
		
		We now provide an example where the Gauss-Green formula fails if $f, \varphi \in \dirichlet_0.$ We use the example in \cite{Barlow:RWHK}. We consider the canonical network on $\N$ and we choose $\varphi = 1$ and $\ds f(n) = \sum_{k = 1}^n \frac{(-1)^k}{k}.$ Define $\ds \varphi_j = \indic{\{1, \ldots, j\}} + \sum_{k = 1}^j \frac{j - k}{j} \indic{\{k\}}$ and $f_j = f \indic{\{1, \ldots, j\}},$ is is easy to see that $\varphi_j \to \varphi$ and $f_j \to f$ in $\dirichlet$ and since $\varphi_j, f_j$ have finite support, both $f$ and $\varphi$ belong to $\dirichlet_0.$ Now, $(f - Pf)(k) = (-1)^{k + 1} \left[ \dfrac{k + \frac{1}{2}}{k(k + 1)} \right]$ and so, the inner-product $\prodEsc{f - Pf}{\varphi}$ converges conditionally (compare with $\dfrac{(-1)^k}{k}$). Since $\nabla \varphi = 0,$ the left hand side is absolutely convergent to zero, thus Gauss-Green formula fails.
	\end{proof}
	
	Observe that $\dirichlet_0$ is the closure of the span of the functions $\indic{x},$ where $x$ is a vertex. Now, a direct calculation shows,
	\begin{equation}
		\nabla \indic{x} = \sum_{e^- = x} c(e) \chi^e,
	\end{equation}
	which amounts to saying that the gradient of $\indic{x}$ is the star at $x.$ Therefore, since $\nabla:\dirichlet \to \ell_-^2(\strE; r)$ is continuous,
	\begin{equation}\label{Equation: The gradient of D0 is the stars}
		\nabla(\dirichlet_0) = \bigstar.
	\end{equation}
	
	\begin{Proposition}\label{Proposition: The Greens function belongs to D0}
		For every vertex $x,$ the function $\ds G_x = \sum_{n = 0}^\infty P^n \indic{x}$ (\ref{Proposition: Properties of the transition operator}) belongs to $\dirichlet_0.$ Thus, for every finitely supported function $\varphi,$ we have $\ds \sum_{n = 0}^\infty P^n \varphi \in \dirichlet_0.$
	\end{Proposition}
	\begin{proof}
		The second claim follows from the first for we have for such $\varphi,$
		\begin{displaymath}
			\sum_{n = 0}^\infty P^n\varphi = \sum_{x \in \strS} \varphi(x) \sum_{n = 0}^\infty P^n \indic{x},
		\end{displaymath}
		where $\strS$ is the support of $\varphi.$
		
		It remains to show that $\ds \sum_{n = 0}^\infty P^n\indic{x} \in \dirichlet_0$ for every $x \in \strV.$ By (\ref{Proposition: Properties of the transition operator}) and Lebesgue-Tonelli's thereom, with $(S_n)$ the network random walk,
		\begin{displaymath}
			G_x(y) = \sum_{n = 0}^\infty \Expectation[^y]{\indic{x}(S_n)} = \Expectation[^y]{ \sum_{n = 0}^\infty \indic{x}(S_n) }.
		\end{displaymath}
		Consider $\tau_k = \tau_{\strV \setminus \strV_k}$ the exit time of $\strV_k$ ($k \geq 1$) by the random walk, and set
		\begin{displaymath}
			G_{x, k}(y) = \sum_{n = 0}^\infty \Expectation[^y]{ \indic{x}(S_n) \indic{ \{\tau_k > n\} } } = \Expectation[^y]{ \sum_{n = 0}^\infty \indic{x}(S_n) \indic{ \{\tau_k > n\} } }.
		\end{displaymath}
		Then $G_{x, k} \to G_x,$ simply, by virtue of the monotone convergence theorem. If $x \notin \strV_k$ or $y \notin \strV_k,$ then $G_{x, k}(y) = 0$ and each $G_{x, k} \in \compactSupp[_\R]{\strV} \subset \ell^2(\strV; c) \subset \dirichlet_0.$ By the Gauss-Green formula (\ref{Proposition: Gauss Green for finite support and dirichlet functions}), for $N \in \N$ and $m \in \Z_+,$
		\begin{displaymath}
			\prodEsc{\nabla G_{x, N}}{\nabla G_{x, N + m}}_{\ell_-^2(\strE; r)} = \prodEsc{G_{x, N}}{G_{x, N + m} - PG_{x, N + m}}_{\ell^2(\strV; c)}.
		\end{displaymath}
		Since $G_{x, N}$ has support contained in $\strV_N,$ the only values that matter are $G_{x, N}(y)$ and $G_{x, N + m}(y) - PG_{x, N + m}(y)$ for $y \in \strV_N.$ By first-step  analysis (for $y \in \strV_N$)
		\begin{displaymath}
			G_{x, N + m}(y) - PG_{x, N + m}(y) = \indic{x}(y).
		\end{displaymath}
		Therefore,
		\begin{displaymath}
			\prodEsc{\nabla G_{x, N}}{\nabla G_{x, N + m}}_{\ell_-^2(\strE; r)} = \sum_{y \in \strV_N} c(y) G_{x, N}(y) \indic{x}(y) = c(x) G_{x, N}(x).
		\end{displaymath}
		With this in mind,
		\begin{align*}
			\energyDir{G_{x, N} - G_{x, N + m}} &= \energyDir{G_{x, N}} + \energyDir{G_{x, N + m}} - 2\prodEsc{\nabla G_{x, N}}{\nabla G_{x, N + m}}_{\ell_-^2(\strE; r)} \\
			&= c(x) G_{x, N}(x) + c(x) G_{x, N + m}(x) - 2 c(x) G_{x, N}(x) \\
			&= c(x) \big( G_{x, N + m}(x) - G_{x, N}(x) \big).
		\end{align*}
		Since $G_{x, k}(y) \to G_x(y)$ for every $y,$ $(G_{x, k})_{k \in \N}$ is a fundamental sequence in $\dirichlet_0,$ and therefore converges to some limit $H \in \dirichlet_0,$ but evaluation is continuous by (\ref{Proposition: Evaluation is a continuous linear function on the Dirichlet space}) and so $H = G_x,$ as claimed.
	\end{proof}
	
	\begin{Proposition}\label{Proposition: Characterisation of the convergence in Dirichlet0 as that of the positive and negative parts}
		In order that $f \in \dirichlet_0,$ it is necessary and sufficient that $f^+$ and $f^-$ should belong to $\dirichlet_0.$ Furthermore, for $f$ to belong to $\dirichlet_0$ it is necessary and sufficient that there should exist two sequences $(s_n)$ and $(t_n)$ of functions with finite support such that $0 \leq s_n \leq f^+,$ $0 \leq t_n \leq f^-$ and $s_n \to f^+,$ $t_n \to f^-$ in the topology of $\dirichlet.$
	\end{Proposition}
	\begin{proof}
		We know that $f \in \dirichlet_0$ if and only if $f_n \to f$ in the topology of $\dirichlet$ for some sequence of functions with finite support. For such a sequence, it is clear that $f_n^\pm$ have finite support and by (\ref{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}), we have that $f_n^\pm \to f^\pm,$ showing that both $f^\pm \in \dirichlet_0;$ the converse is obvious since $f = f^+ - f^-.$ We prove now the second claim, the sufficiency is obvious for then $f^+$ and $f^-$ belong to $\dirichlet_0.$ We prove the necessity. Since $f \in \dirichlet_0,$ there is a sequence $(f_n)$ of functions with finite support such that $f_n \to f$ in $\dirichlet.$ Then $f_n^\pm \to f^\pm$ in $\dirichlet$ by (\ref{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}). Consider $s_n = \min(f_n^+, f^+)$ and $t_n = \min(f_n^-, f^-).$ Clearly $0 \leq s_n \leq f^+,$ $0 \leq t_n \leq f^-$ and $s_n(o) \to f^+(o), t_n(o) \to f^-(o).$ By (\ref{Proposition: The Dirichlet energy of the difference of two functions is greater than the Dirichlet energy of the difference of any of them minus its minimum}), $\energyDir{s_n - f^+} \leq \energyDir{f_n^+ - f^+}$ and $\energyDir{t_n - f^-} \leq \energyDir{f_n^- - f^-},$ showing the claim by (\ref{Proposition: Characterisation of the topology in the Dirichlet space}).
	\end{proof}

	Using $\dirichlet_0,$ we may now provide another version of Dirichlet's principle.
	\begin{Proposition}\label{Proposition: Dirichlets principle from a vertex to infinity, D0 case}
		Let $o$ be a vertex of a network $\Gamma$ satisfying the usual assumptions. Then
		\begin{displaymath}
			\effCon{o, \infty} = \inf_{\substack{\varphi \in \dirichlet_0 \\ \varphi(o) = 1}} \energyDir{\varphi},
		\end{displaymath}
		(``Dirichlet's principle'').
	\end{Proposition}
	\begin{proof}
		By (\ref{Equation: Dirichlet principle from a vertex to infinity, finite support}), we have
		\begin{displaymath}
			\effCon{o, \infty} = \inf \energyDir{\varphi},
		\end{displaymath}
		where $\varphi(o) = 1$ and $\varphi$ has finite support; such $\varphi$ is a Dirichlet function. Consider $\strZ_0$ (respectively $\strZ$) to be the set of $\varphi$ with finite support (respectively that belongs to $\dirichlet_0$) such that $\varphi(o) = 1$ and denote by $\closure{\strZ}_0$ its closure in $\dirichlet.$ Then $\strZ = e_o^{-1}(\{1\}),$ where $e_o:\dirichlet_0 \to \R$ is the evaluation $\varphi \mapsto \varphi(o);$ since $e_o$ is continuous (\ref{Proposition: Evaluation is a continuous linear function on the Dirichlet space}), $\strZ$ is closed. Clearly $\strZ_0 \subset \strZ,$ hence $\closure{\strZ}_0 \subset \strZ.$ Now, if $\varphi \in \strZ$ there exists a sequence $\psi_n$ of functions with finite support such that $\psi_n \to \varphi$ in $\dirichlet,$ define $\varphi_n = \psi_n + (1 - \psi_n(o)) \indic{o}.$ Clearly $\varphi_n(o) = 1,$ so $\varphi_n \in \strZ_0,$ and
		\begin{displaymath}
			\norm{\varphi - \varphi_n}_o \leq \norm{\varphi - \psi_n}_o + |1 - \psi_n(o)| \norm{\indic{o}}_o \to 0,
		\end{displaymath}
		showing that $\varphi \in \closure{\strZ}_0.$ Hence $\strZ = \closure{\strZ}_0.$ So, the claim that
		\begin{displaymath}
			\inf_{\varphi \in \strZ_0} \energyDir{\varphi} = \inf_{\varphi \in \strZ} \energyDir{\varphi}
		\end{displaymath}
		is now obvious since $\energyDir{\cdot}$ is continuous $\dirichlet \to \R.$
	\end{proof}

	\section{The Hilbert space $\dirichlet/\R.$}
	Consider now the quotient set $\dirichlet/\R,$ that is, two Dirichlet functions are identified if its difference is a constant function. Define on the set $\dirichlet/\R \times \dirichlet/\R$ the following function
	\begin{equation}\label{Equation: Definition of the inner product in the quotient Dirichlet space}
		\left( \tilde{f}, \tilde{g} \right) \mapsto \prodEsc{\tilde f}{\tilde g}_{\dirichlet/\R} = \prodEsc{\nabla f}{\nabla g}_{\ell_-^2(\strE; r)},
	\end{equation}
	where $f \in \tilde{f}$ and $g \in \tilde{g},$ this is well-defined by (\ref{Proposition: A function is constant iff its energy is zero}). This defines on $\dirichlet/\R$ a structure of Hilbert space. This easily follows from the the characterisation of the topology of $\dirichlet$ (\ref{Proposition: Characterisation of the topology in the Dirichlet space}). If $\left( \tilde f_n \right)$ is a fundamental sequence in $\dirichlet/\R,$ then we can choose representatives $f_n \in \tilde f_n$ for which $f_n(o) = 0$ and so $(f_n)$ is fundamental in $\dirichlet$ with respect to $\norm{ \cdot }_o$ and it therefore converges to a function $f \in \dirichlet,$ which satisfies $\energyDir{f_n - f} \to 0.$ Then $\tilde f$ is the limit of $\left( \tilde f_n \right).$
	
	We transport now the definition of $\nabla$ from being a function $\dirichlet \to \ell_-^2(\strE; r)$ to a function $\dirichlet/\R \to \ell_-^2(\strE; r)$ by setting $\nabla \tilde f = \nabla f$ for any $f \in \tilde f.$
	\begin{Proposition}\label{Proposition: The gradient is an isomorphism between the classes of Dirichlet functions and the orthogonal space to the cycles}
		The function $\nabla:\dirichlet/\R \to \ell_-^2(\strE; r)$ has image $\lozenge^\perp$ and $\nabla:\dirichlet/\R \to \lozenge^\perp$ is an isomorphism of Hilbert spaces (it is a bijection that preserves inner product).
	\end{Proposition}
	\begin{proof}
		By (\ref{Proposition: The orthogonal space to the cycles are the flows with potential}), $\nabla \tilde f \in \lozenge^\perp$ and reciprocally, a flow in $\lozenge^\perp$ is of the form $\nabla f = \nabla \tilde f,$ where $f \in \dirichlet$ and $\tilde f$ is the class of $f.$ Hence, all reduces to show that $\nabla:\dirichlet/\R \to \lozenge^\perp$ is an isomorphism of Hilbert spaces. It follows immediately from (\ref{Equation: Definition of the inner product in the quotient Dirichlet space}) that $\nabla$ preserves inner product and therefore, it also preserves the norm, that is, $\norm{\nabla \tilde f}_{\dirichlet/\R} = \norm{\nabla f}_{\ell_-^2(\strE; r)}$ and so, $\nabla:\dirichlet/\R \to \lozenge^\perp$ is bijective and this completes the proof.
	\end{proof}
	
	Denote now by $\tilde \dirichlet_0$ the set of classes $\tilde f$ as $f$ runs through $\dirichlet_0.$ Since the operator $\nabla:\dirichlet/\R \to \lozenge^\perp$ is an isomorphism of Hilbert spaces (\ref{Proposition: The gradient is an isomorphism between the classes of Dirichlet functions and the orthogonal space to the cycles}), and $\lozenge^\perp = \bigstar \oplus \nabla \harDirichlet$ is an orthogonal decomposition of $\lozenge^\perp$ by (\ref{Theorem: Decomposition of the space of flows}), it follows that $\dirichlet/\R = \nabla^{-1} (\bigstar) \oplus \harDirichlet/\R$ is an orthogonal decomposition. Upon applying the equivalence relation, the equality $\nabla(\dirichlet_0) = \bigstar$ (\ref{Equation: The gradient of D0 is the stars}) is the same as saying $\tilde \dirichlet_0 = \nabla^{-1} (\bigstar).$ We have therefore an orthogonal decomposition of the Hilbert space $\dirichlet/\R$
	\begin{equation}
		\dirichlet/\R = \tilde \dirichlet_0 \oplus \harDirichlet/\R.
	\end{equation}
	An immediate corollary of this decomposition is that $\dirichlet_0 \cap \harDirichlet$ is contained in the set of constant functions. This intersection reduces to $\{0\}$ in many cases as the next proposition shows.
	
	\begin{Proposition}\label{Proposition: Characterisation of recurrence as using Dirichlet functions with finite support}
		The following three conditions are equivalent on network $\Gamma$ satisfying the usual assumptions.
		\begin{enumerate}\renewcommand{\labelenumi}{(\alph{enumi})}
			\item $\dirichlet_0$ contains the constant functions;
			\item $\dirichlet_0 = \dirichlet;$
			\item the network random walk in $\Gamma$ is recurrent.
		\end{enumerate}
	\end{Proposition}
	\begin{proof}
		We know that $\dirichlet_0 \subset \dirichlet$ always and it is obvious that condition (b) implies condition (a). We now prove that $1 \in \dirichlet_0$ is sufficient for $\dirichlet_0 = \dirichlet,$ so assume $1 \in \dirichlet_0.$ Since $1 \in \dirichlet_0,$ there exists a sequence $f_n$ of functions with finite support such that $f_n \to 1$ in the topology of $\dirichlet.$ Since $1$ is already its positive part, we may assume $f_n$ to be positive as well (\ref{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}). By passing through a subsequence (also denoted by $(f_n)$), we may assume $\norm{f_n - 1}_o \leq n^{-2}.$ Introduce $g_n = nf_n,$ which are also non-negative and finitely supported functions. Then
		\begin{displaymath}
			\energyDir{g_n} = n^2 \energyDir{f_n} \leq n^2 n^{-4} = n^{-2},
		\end{displaymath}
		and $g_n(v) \to \infty$ for every vertex $v$ since $f_n(v) \to 1$ and evaluation is continuous (\ref{Proposition: Evaluation is a continuous linear function on the Dirichlet space}).
		
		Given $u \in \dirichlet,$ we have $u = u^+ - u^-$ with both $u^\pm \in \dirichlet$ (\ref{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}) and so, suffices to show every non-negative Dirichlet function belongs to $\dirichlet_0.$ For such a function $u,$ set the sequence $(u_n)$ by $u_n = \min(u, g_n).$ Then, $u_n$ is a sequence of non negative and finitely supported functions such that for every vertex $x,$ there is an index $n_x$ such that $u_n(x) = u(x)$ for all $n \geq n_x.$ Consider $\strE_n$ to be the set of edges $e$ for which $\nabla u(e) \neq \nabla u_n(e).$ Since the network is denumerable, we may order the vertex set $\strV = (v_j)_{j \in \N}.$ For every positive integer $J$ there exists $n_J \in \N$ such that for all $n \geq n_J,$ no edge joining vertices among $\avec{v}{1}{J}$ will be in $\strE_n.$ Then, $\ds \sum_{e \in \strE_n} \dfrac{1}{2} r(e) \nabla u(e)^2$ can be made arbitrarily small if $n$ is large enough, that is to say, $\ds \sum_{e \in \strE_n} \dfrac{1}{2} r(e) \nabla u(e)^2 = \littleO{1}$ as $n \to \infty.$ By definition of $\strE_n,$
		\begin{displaymath}
			\norm{u - u_n}_o^2 = \sum_{e \in \strE_n} \dfrac{1}{2} r(e) \big( \nabla u(e) - \nabla u_n(e) \big)^2.
		\end{displaymath}
		By (\ref{Proposition: The Dirichlet energy of the difference of two functions is greater than the Dirichlet energy of the difference of any of them minus its minimum}),
		\begin{displaymath}
			|u(e^+) - u(e^-) - u_n(e^+) + u_n(e^-)|^2 \leq 2 |u(e^+) - u(e^-)|^2 + 2|g_n(e^+) - g_n(e^-)|^2,
		\end{displaymath}
		and this bound implies
		\begin{displaymath}
			\big( \nabla u(e) - \nabla u_n(e) \big)^2 \leq 2 \nabla u(e)^2 + 2 \nabla g_n(e)^2.
		\end{displaymath}
		Therefore
		\begin{displaymath}
			\norm{u - u_n}_o^2 \leq \sum_{e \in \strE_n} r(e) \nabla u(e)^2 + \sum_{e \in \strE_n} r(e) \nabla g_n(e)^2 \leq \littleO{1} + 2n^{-2} = \littleO{1}
		\end{displaymath}
		as $n \to \infty.$ Thus, showing $\dirichlet = \dirichlet_0$ as desired. 
		
		It remains to show that (c) is equivalent to (b). For this, observe that by (\ref{Proposition: Dirichlets principle from a vertex to infinity, D0 case})
		\begin{align*}
			\norm{1 - \dirichlet_0}_{\dirichlet}^2 &=  \inf\{\norm{1 - f}_o^2: f \in \dirichlet_0\} \\
			&\leq \inf\{\norm{1 - f}_o^2: f \in \dirichlet_0, f(o) = 1\} = \effCon{o, \infty},
		\end{align*}
		with equality if the constant functions belong to $\dirichlet_0,$  Therefore, we have established
		\begin{displaymath}
			\norm{1 - \dirichlet_0}_{\dirichlet}^2 \leq \effCon{o, \infty},
		\end{displaymath}
		with  equality if $1 \in \dirichlet_0.$ We may now apply Doyle and Snell's criterion (\ref{Proposition: Doyle and Snells criterion}). Then, $1 \in \dirichlet_0$ if the network is recurrent since then $\effCon{o, \infty} = 0,$ and if $1 \notin \dirichlet_0$ then $\effCon{o, \infty} > 0$ and the network is transient. This concludes the proof.
	\end{proof}

	\section{Riesz' and Royden's decompositions.}
	By the previous proposition, when the network random walk in $\strG$ is transient, $\dirichlet_0 \cap \harDirichlet = \{0\}$ and we have the following decomposition as a direct sum
	\begin{displaymath}
		\dirichlet = \dirichlet_0 + \harDirichlet.
	\end{displaymath}
	Therefore, in the transient case, every function $f \in \dirichlet$ is uniquely expressible as
	\begin{equation}\label{Equation: Royden decomposition}
		f = f_{\dirichlet_0} + f_{\harDirichlet},
	\end{equation}
	where $f_{\dirichlet_0} \in \dirichlet_0$ and $f_{\harDirichlet} \in \harDirichlet$ (``Royden's decomposition''). Observe that in general $f_{\dirichlet_0}$ and $f_{\harDirichlet}$ are not orthogonal vectors in $\dirichlet,$ even when $\nabla f_{\dirichlet_0}$ is orthogonal to $\nabla f_{\harDirichlet},$ for
	\begin{displaymath}
		\prodEsc{f_{\dirichlet_0}}{f_{\harDirichlet}}_o = f_{\dirichlet_0}(o) f_{\harDirichlet}(o).
	\end{displaymath}
	
	We recall the definition of superharmonic function as a function $f:\strV \to \R$ such that $Pf \leq f.$ If $(S_n)_{n \in \Z_+}$ is the network random walk with $S_0$ constant, then $(Pf(S_n))_{n \in \Z_+}$ defines a supermartingale, as it is easily seen from definitions (proof is identical to (\ref{Proposition: A harmonic function of a SRW is a martingale})).
	
	\begin{Proposition}\label{Proposition: The superharmonic functions in D0 are non negative}
		Consider a network satisfying the usual assumptions $\Gamma.$ The superharmonic functions in $\dirichlet_0$ are necessarily non-negative.
	\end{Proposition}
	\begin{proof}
		Suppose $f \in \dirichlet_0$ is superharmonic. Observe that $\energyDir{|f|} \leq \energyDir{f}$ (\ref{Proposition: Lipschitz functions preserve Dirichlet functions}) and that $|f| = f + 2f^-,$ this last equality implies
		\begin{displaymath}
			\energyDir{|f|} = \energyDir{f} + 4\energyDir{f^-} + 4 \prodEsc{\nabla f}{\nabla f^-}_{\ell_-^2(\strE; r)}.
		\end{displaymath}
		Consider $f_n$ having finite support and $f_n \to f$ in $\dirichlet,$ then $f_n^- \to f^-$ in $\dirichlet$ by (\ref{Proposition: Characterisation of the convergence in the Dirichlet space as the convergence of the positive and negative parts}). Hence, by the Gauss-Green formula (\ref{Proposition: Gauss Green for finite support and dirichlet functions}),
		\begin{displaymath}
			\prodEsc{\nabla f}{\nabla f^-}_{\ell_-^2(\strE; r)} = \lim_{n \to \infty} \prodEsc{\nabla f}{\nabla f_n^-}_{\ell_-^2(\strE; r)} = \lim_{n \to \infty} \prodEsc{f - Pf}{f_n^-}_{\ell^2(\strV; c)} \geq 0
		\end{displaymath}
		since $f - Pf \geq 0.$ Whence, $\energyDir{f} \leq \energyDir{|f|}$ and therefore, $\energyDir{f} = \energyDir{|f|}$ and $\energyDir{f^-} = 0.$ This shows that $f^-$ is a constant function. Since $f^- \in \dirichlet_0,$ it follows from (\ref{Proposition: Characterisation of recurrence as using Dirichlet functions with finite support}) that $f^- = 0.$ Thus, $f = f^+ \geq 0.$
	\end{proof}

	\begin{Proposition}\label{Proposition: Riesz decomposition in transient networks}
		Suppose $\Gamma$ is a network satisfying the usual assumptions.  Every non-negative superharmonic function $f$ is uniquely expressible as $\ds f = \sum_{n = 0}^\infty P^nu + h,$ where $u$ is non-negative and $h$ is harmonic (``Riesz' decomposition''); in this decomposition, $h \geq 0.$
	\end{Proposition}
	\begin{proof}
		The superharmonicity of $f$ implies that $(P^n f)$ is non-increasing and therefore, since $f \geq 0,$ the sequence of functions $P^n f$ converges simply to a function $h.$ We will show $h$ is harmonic. Clearly $f - P^n f \uparrow f - h,$ thus the monotone convergence theorem shows that, for every $x \in \strV,$
		\begin{displaymath}
			\lim_{n \to \infty} P(f - P^n f)(x) = P(f - h)(x).
		\end{displaymath}
		Since $0 \leq Pf(x) \leq f(x),$ we have $\ds \lim_{n \to \infty} P^{n + 1} f(x) \to Ph(x).$ Thus $h(x) = Ph(x),$ that is to say, $h$ is harmonic at $x.$ Consider now $u = f - Pf \geq 0.$ Then, $\ds \sum_{n = 0}^N P^n u = f - P^N f$ and taking the limit as $N \to \infty,$ the right hand side converges simply to $f - h,$ and by definition, the left hand side converges and its limit is $\ds \sum_{n = 0}^\infty P^n u.$ The decomposition has been established. We now prove this decomposition is unique. If $\ds \sum_{n = 0}^\infty P^n u_1 + h_1 = \sum_{n = 0}^\infty P^n u_2 + h_2$ are two decompositions of $f,$ we may apply Lebesgue's convergence theorem to show, for every $x \in \strV,$
		\begin{displaymath}
			P\left( \sum_{n = 0}^\infty P^n (u_2 - u_1) \right)(x) = \sum_{n = 0}^\infty P^{n + 1} (u_2 - u_1)(x).
		\end{displaymath}
		However,
		\begin{displaymath}
			\sum_{n = 0}^\infty P^n (u_2 - u_1) = h_1 - h_2 = P(h_1 - h_2) = \sum_{n = 0}^\infty P^{n + 1} (u_2 - u_1).
		\end{displaymath}
		Thus, $u_2 - u_1 = 0$ and then $h_1 - h_2 = 0$ as well.
	\end{proof}

	\begin{Proposition}\label{Proposition: Riesz decomposition of a superharmonic function in D0}
		The Riesz decomposition for a superharmonic function $f$ in $\dirichlet_0$ is of the form $\ds f = \sum_{n = 0}^\infty P^n u$ where $u \geq 0.$
	\end{Proposition}
	\begin{proof}
		The Riesz decomposition of $f$ exists (\ref{Proposition: Riesz decomposition in transient networks}) and we may write $\ds f = \sum_{n = 0}^\infty P^n u + h,$ where $u \geq 0$ and $h \geq 0$ is harmonic. Consider now an exhaustion $(\strG_k)$ of $\strG$ and let $\strV_k$ be the vertex set of $\strG_k.$ The exhaustion is chosen so that each $\strV_k$ is finite. Set $\ds u_k = u \indic{\strV_k}$ and $\ds f_k = \sum_{n = 0}^\infty P^n u_k,$ notice that $u_k$ belongs to $\dirichlet_0$ having finite support and so, $f_k \in \dirichlet_0$ as well (\ref{Proposition: The Greens function belongs to D0}). Consider now a sequence of functions $0 \leq f_{k, n} \leq f_k$ having finite support and $f_{k, n} \to f_k$ in $\dirichlet$ (\ref{Proposition: Characterisation of the convergence in Dirichlet0 as that of the positive and negative parts}). Then, $\nabla f_{k, n} \to \nabla f_k$ in $\ell_-^2(\strE; r);$ therefore, using the Gauss-Green formula (\ref{Proposition: Gauss Green for finite support and dirichlet functions})
		\begin{displaymath}
			\energyDir{f_k} = \lim_{n \to \infty} \prodEsc{\nabla f_k}{\nabla f_{k, n}}_{\ell_-^2(\strE; r)} = \lim_{n \to \infty} \prodEsc{f_k - Pf_k}{f_{k, n}}_{\ell^2(\strV; c)}.
		\end{displaymath}
		Now, $f_k - Pf_k = u_k \geq 0,$ and clearly $u_k \leq u = f - Pf \in \ell^2(\strV; c)$ by (\ref{Proposition: I-P maps D into L2}), hence
		\begin{displaymath}
			\prodEsc{f_k - Pf_k}{f_{k, n}}_{\ell^2(\strV; c)} \leq \prodEsc{f - Pf}{f_{k, n}}_{\ell^2(\strV; c)}.
		\end{displaymath}
		Using again the Gauss-Green formula, it follows that
		\begin{displaymath}
			\prodEsc{f - Pf}{f_{k, n}}_{\ell^2(\strV; c)} = \prodEsc{\nabla f}{\nabla f_{k, n}}_{\ell_-^2(\strE; r)} \leq \energyDir{f}^{\frac{1}{2}} \energyDir{f_{k, n}}^{\frac{1}{2}}.
		\end{displaymath}
		Whence, we proved that
		\begin{displaymath}
			\energyDir{f_k} \leq \lim_{n \to \infty} \energyDir{f}^{\frac{1}{2}} \energyDir{f_{k, n}}^{\frac{1}{2}} = \energyDir{f}^{\frac{1}{2}} \energyDir{f_k}^{\frac{1}{2}},
		\end{displaymath}
		which in turn implies $\energyDir{f_k} \leq \energyDir{f}$ (since $\energyDir{f_k} < \infty$).
		
			Thus far, we have constructed the functions $u_k = u \indic{\strV_k}$ and $\ds f_k = \sum_{n = 0}^\infty P^n u_k \in \dirichlet_0$ and showed that $\energyDir{f_k} \leq \energyDir{f}.$ Observe that the monotone convergence theorem shows $\ds \lim_{k \to \infty} f_k(x) = \sum_{n = 0}^\infty P^n u(x)$ for every vertex $x \in \strV.$ By Fatou's lemma,
			\begin{displaymath}
				\energyDir{\sum_{n = 0}^\infty P^n u} \leq \liminf_{k \to \infty} \energyDir{\sum_{n = 0}^\infty P^n u_k} = \liminf_{k \to \infty} \energyDir{f_k} \leq \energyDir{f} < \infty.
			\end{displaymath}
			Hence, in the Riesz decomposition of $\ds f = \sum_{n = 0}^\infty P^n u + h,$ we proved that $\ds \sum_{n = 0}^\infty P^n u \in \dirichlet$ and so, $h \in \harDirichlet.$ Then, if we can show that $\ds \sum_{n = 0}^\infty P^n u \in \dirichlet_0,$ the Riesz decomposition of $f$ will also be the Royden's decomposition by uniqueness. Having this and the fact $f$ already belongs to $\dirichlet_0,$ will show together that $h = 0,$ which is the desired conclusion. All reduces to show that $\ds \sum_{n = 0}^\infty P^n u \in \dirichlet_0.$
		
			We now prove that $\ds \sum_{n = 0}^\infty P^n u \in \dirichlet_0$ and this will terminate the proposition. To begin with, $\norm{f_k}_o \leq \norm{f}_o$ and therefore, $f_k$ lies in $\ball[_{\dirichlet_0}]{0; \norm{f}_o}$ the ball of centre zero and radius $\norm{f}_o$ in the Hilbert space $\dirichlet_0.$ Remark from (\ref{Equation: The gradient of D0 is the stars}) that $\nabla(\dirichlet_0) = \bigstar$ and that $\nabla:\dirichlet_0 \to \bigstar$ is continuous by (\ref{Equation: The gradient is continuous from the Dirichlet into the flows}). Now, $\nabla:\dirichlet_0 \to \bigstar$ is injective for if $\nabla f = 0$ for some $f \in \dirichlet_0$ then $f$ is a constant function on $\strV,$ but the network random walk is transient by hypothesis, showing that there are no constant functions in $\dirichlet_0$ other than the function zero (\ref{Proposition: Characterisation of recurrence as using Dirichlet functions with finite support}), thus $f = 0$ and $\nabla$ is injective as claimed. Whence, $\nabla:\dirichlet_0 \to \bigstar$ is a continuous linear bijection between Hilbert spaces. Taking advantage of Banach-Schauder theorem, $\nabla:\dirichlet_0 \to \bigstar$ has a continuous inverse. Since $\bigstar$ is separable (\ref{Proposition: Separability of the space of flows with finite energy}), $\dirichlet_0$ is also separable. By invoking Banach-Alaoglu theorem, we see that $\ball[_{\dirichlet_0}]{0; \norm{f}_o}$ is a metrisable compact space in the weak topology of $\dirichlet_0.$ Thus, $(f_k)$ has limit points in $\ball[_{\dirichlet_0}]{0; \norm{f}_o}$ relative to the weak topology. But we know that evaluation is a continuous linear form $\dirichlet_0 \to \R$ (\ref{Proposition: Evaluation is a continuous linear function on the Dirichlet space}), and we already proved that $\ds f_k(x) \to \sum_{n = 0}^\infty P^n u(x),$ this entails that $\ds \sum_{n = 0}^\infty P^n u$ is a limit point of $(f_k)$ (in fact, the unique limit point). Henceforth, $\ds \sum_{n = 0}^\infty P^n u \in \dirichlet_0$ as desired.
		\end{proof}

	\section{The space $\harDirichlet$ and the Dirichlet Liouville property.}
	Recall from Chapter \ref{Chapter: Liouville property on the network, WSF = FSF, Number of trees} that the Dirichlet Liouville property ($\mathsf{DLP}$) states that any Dirichlet harmonic function is constant, while the Liouville propery ($\mathsf{LP}$), any bounded harmonic function is constant. We are going to show $(\mathsf{LP}) \implies (\mathsf{DLP}).$ As such, we need a few more tools regarding $\harDirichlet.$

	\begin{Proposition}
		Suppose the network random walk on a network satisfying the usual assumptions is transient. Denote by $\harDirichlet_+$ the set of harmonic Dirichlet functions that are non negative. Then $\harDirichlet = \harDirichlet_+ - \harDirichlet_+.$
	\end{Proposition}
	\begin{proof}
		Consider $f \in \harDirichlet$ and decompose $f = f^+ - f^-.$ We know that $f^\pm \in \dirichlet$ and by virtue of Royden's decomposition, $f^\pm$ is uniquely expressible as $f^\pm = v_\pm + u_\pm$ with $v_\pm \in \dirichlet_0$ and $u_\pm \in \harDirichlet.$ It is easy to check that $Pf^\pm \geq f^\pm$ and since $Pu_\pm = u_\pm$ for $i = 1, 2,$ it follows that $Pv_\pm \geq v_\pm.$  Hence, $-v_\pm$ are superharmonic functions in $\dirichlet_0,$ and therefore $-v_\pm \geq 0$ by (\ref{Proposition: Riesz decomposition in transient networks}). Since $f^\pm = v_\pm + u_\pm \geq 0,$ we get $u_\pm \geq -v_\pm \geq 0$ and thus $u_\pm$ are non-negative harmonic functions. Finally, $f = f^+ - f^- = (v_+ - v_-) + (u_+ - u_-)$ and since $f$ has a unique Royden's decomposition, if follows that $v_+ - v_- = 0$ and so $f = u_+ - u_-$ is the difference of two non-negative harmonic Dirichlet functions as desired.
	\end{proof}
	
	\begin{Proposition}\label{Proposition: Bounded harmonic functions are dense in HD}
		The bounded harmonic Dirichlet functions are dense in $\harDirichlet;$ in fact, the set of bounded functions in $\harDirichlet_+$ is a dense subset on $\harDirichlet_+.$
	\end{Proposition}
	\begin{proof}
		The proposition will be completely proven if we show the second claim. Indeed, any $f \in \harDirichlet$ can be written as $f = f_1 - f_2$ with both $f_1$ and $f_2$ positive harmonic Dirichlet functions, as proven in the previous proposition.  Given $f \in \harDirichlet_+,$ consider $f_n = \min(f, n),$ which is readily seen to be superharmonic. Royden's decomposition allows expressing uniquely
		\begin{displaymath}
			f_n = u_n + h_n,
		\end{displaymath}
		where $u_n \in \dirichlet_0$ and $h_n \in \harDirichlet.$ Since $f_n$ is superharmonic and $h_n$ harmonic, $u_n$ is superharmonic as well, and as $u_n \in \dirichlet_0,$ it follows that $u_n$ is a non negative (\ref{Proposition: The superharmonic functions in D0 are non negative}) and $\ds u_n = \sum_{m = 0}^\infty P^mv_n$ for some $v_n \geq 0$ (\ref{Proposition: Riesz decomposition of a superharmonic function in D0}). Then $f_n = u_n + h_n$ is also the Riesz decomposition of $f$ and so $h_n \geq 0$ (\ref{Proposition: Riesz decomposition in transient networks}). Now,
		\begin{displaymath}
			\energyDir{f - f_n} = \energyDir{u_n} + \energyDir{f - h_n} - 2 \prodEsc{\nabla u_n}{\nabla (f - h_n)}_{\ell_-^2(\strE; r)} = \energyDir{u_n} + \energyDir{f - h_n},
		\end{displaymath}
		since $\nabla u_n \in \bigstar$ and $\nabla(f - h_n) \in \nabla \harDirichlet.$ By Lebesgue's dominated convergence theorem, $\energyDir{f - f_n} \to 0,$ and therefore $\energyDir{u_n} \to 0$ and $\energyDir{f - h_n} \to 0.$ Since $0 \leq u_n \leq f_n \leq f$ and using a subsequence should the need arise, $(u_n(o))$ can be assumed to converge in $\R$ to some constant $\lambda.$ Therefore, $u_n(o) \to \lambda$ and $\energyDir{u_n} \to 0,$ which together imply that $u_n$ converges in $\dirichlet_0$ to the constant function $\lambda,$ this function belongs to $\dirichlet_0$ since this is a closed subspace. Since the network random walk is assumed transient, the only constant function in $\dirichlet_0$ is the zero function (\ref{Proposition: Characterisation of recurrence as using Dirichlet functions with finite support}), therefore $\lambda = 0.$ Since $f_n(o) = f(o)$ for all large values of $n,$ we deduce that $h_n(o) \to f(o)$ and therefore, $h_n \to f$ in $\dirichlet.$
	\end{proof}
	
	This proposition is cornerstone for the following.
	\begin{Proposition}\label{Proposition: Lioville property implies that HD is R}
		If a network satisfying the usual assumption possesses the Lioville property the it also possesses the Dirichlet Liouville property; in other words, $(\mathsf{LP}) \implies (\mathsf{DLP}).$
	\end{Proposition}
	\begin{proof}
		By (\ref{Proposition: Bounded harmonic functions are dense in HD}), every harmonic function $h \in \harDirichlet$ can be approximated in $\dirichlet$ by constant functions. By (\ref{Proposition: Evaluation is a continuous linear function on the Dirichlet space}), $h$ is constant.
	\end{proof}

	That a network satisfies the Dirichlet Liouville property signifies that $\nabla \harDirichlet = \{0\}.$ Thus, and keeping in mind (\ref{Theorem: The WSF and FSF coincide iff HD is the constants}), a sufficient condition for a network satisfying the usual assumptions, whose underlying graph does not possess multiple edges, to satisfy $\WSF = \FSF$ is that the network should possess the Liouville property, this is just a restatement of Theorem (\ref{Theorem: Liouville property implies equality of wired and free uniform spanning forest}).
